System Demo: Tool and Infrastructure for Offensive Language Error Analysis (OLEA) in English

The automatic detection of offensive language is a pressing societal need. Many systems perform well on explicit offensive language but struggle to detect more complex, nuanced, or implicit cases of offensive and hateful language. OLEA is an open-source Python library that provides easy-to-use tools for error analysis in the context of detecting offensive language in English. OLEA also provides an infrastructure for re-distribution of new datasets and analysis methods requiring very little coding.

==> code_examples/installation.tex <==
\begin{lstlisting}[language=Python]
pip install olea
\end{lstlisting}

==> imgs/Plots/category_hc.tex <==
\begin{figure}[ht]\captionsetup{justification=centering}
\includegraphics[width=0.5\textwidth]{imgs/Plots/Plot_w_percents/hc_cat_plot.png}
\caption{Plot of roBERTa predictions \texttt{analyze\char`_on} on the HateCheck Category column. Percent values above the bars represent the percent accuracy for that category}
\centering
 \label{fig:catHCplot-RoBERTa}
\end{figure}

==> imgs/Plots/hc_cat_hatexplain.tex <==
\begin{figure}[ht]\captionsetup{justification=centering}
\includegraphics[width=0.5\textwidth]{imgs/Plots/hc_cat_hatexplain.png}
\caption{Plot of HateXplain predictions \texttt{analyze\char`_on} on the HateCheck Category column. Percent values above the bars represent the percent accuracy for that category}
\centering
 \label{fig:catHCplot-HateXplain}
\end{figure}

==> imgs/Plots/off-roberta-cold.tex <==
\begin{figure}[h]\captionsetup{justification=centering}
\includegraphics[width=0.5\textwidth]{imgs/Plots/off-roberta-cold.png}
\caption{Plot of $analyze\char`_on$ on the offensiveness column}
\centering
 \label{fig:offCOLDplot}
\end{figure}

==> imgs/TextPreprocessing.tex <==
\begin{figure}[b!]\centering\captionsetup{justification=centering}
\includegraphics[width=0.4\textwidth]{imgs/TextPreprocessing.PNG}
\caption{The before and after of a message that has been passed through the \lib{} preprocessing function.}
\centering
 \label{fig:text_preprocessing}
\end{figure}

==> tables/anno_agree_1.tex <==
\begin{table}
\centering
\begin{tabular}{llllll}
Full Agreement vs Partial Agreement & Metrics      & precision          & recall             & f1-score           & support  \\
Full                                & N            & 0.7430939226519337 & 0.5018656716417911 & 0.5991091314031181 & 1072     \\
Full                                & Y            & 0.586687306501548  & 0.8029661016949152 & 0.6779964221824686 & 944      \\
Full                                & macro avg    & 0.6648906145767408 & 0.6524158866683532 & 0.6385527767927933 & 2016     \\
Full                                & weighted avg & 0.6698559039783404 & 0.6428571428571429 & 0.6360484183553535 & 2016     \\
Partial                             & N            & 0.7430939226519337 & 0.5018656716417911 & 0.5991091314031181 & 1072     \\
Partial                             & Y            & 0.586687306501548  & 0.8029661016949152 & 0.6779964221824686 & 944      \\
Partial                             & macro avg    & 0.6648906145767408 & 0.6524158866683532 & 0.6385527767927933 & 2016     \\
Partial                             & weighted avg & 0.6698559039783404 & 0.6428571428571429 & 0.6360484183553535 & 2016    
\end{tabular}
\end{table}
